Potential functions on Grassmannians of planes and cluster transformations

With a triangulation of a planar polygon with $n$ sides, one can associate an integrable system on the Grassmannian of 2-planes in an $n$-space. In this paper, we show that the potential functions of Lagrangian torus fibers of the integrable systems associated with different triangulations glue together by cluster transformations. We also prove that the cluster transformations coincide with the wall-crossing formula in Lagrangian intersection Floer theory.

==> GC_cluster-1+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-1+0_0.pdf}%
}%


==> GC_cluster-1.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 140.495580pt{}%
\kern 206.762990pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{12.000000}{14.400000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-103.381495,70.247790)(-0.500000,-0.500000){\hbox to 0pt{\includegraphics[hiresbb]{\ASYprefix\jobname-1+0_0.pdf}\hss}%
\includemedia[noplaybutton,3Dlights=Headlamp,3Dmenu,3Dtoolbar=false,label=GC_cluster-1,3Daac=17.761892019,3Dc2w=0.613940614 -0.789352217 0 -0.200855944 -0.15622129 0.967084173 -0.763370037 -0.593732251 -0.254456679 383.208941922 309.35148192 160.454625087,3Droo=422.541929331,3Dpsob=H,3Dbg=1 1 1,add3Djscript=asylabels.js]{\phantom{\includegraphics[hiresbb]{\ASYprefix\jobname-1+0_0.pdf}}}{\ASYprefix\jobname-1+0.prc}}%

